Universal Dynamics of Damped-Driven Systems: The Logistic Map as a Normal Form for Energy Balance

Damped-driven systems are ubiquitous in engineering and science. Despite the diversity of physical processes observed in a broad range of applications, the underlying instabilities observed in practice have a universal characterization which is determined by the overall gain and loss curves of a given system. The universal behavior of damped-driven systems can be understood from a geometrical description of the energy balance with a minimal number of assumptions. The assumptions on the energy dynamics are as follows: the energy increases monotonically as a function of increasing gain, and the losses become increasingly larger with increasing energy, i.e. there are many routes for dissipation in the system for large input energy. The intersection of the gain and loss curves define an energy balanced solution. By constructing an iterative map between the loss and gain curves, the dynamics can be shown to be homeomorphic to the logistic map, which exhibits a period doubling cascade to chaos. Indeed, the loss and gain curves allow for a geometrical description of the dynamics through a simple Verhulst diagram (cobweb plot). Thus irrespective of the physics and its complexities, this simple geometrical description dictates the universal set of logistic map instabilities that arise in complex damped-driven systems. More broadly, damped-driven systems are a class of non-equilibrium pattern forming systems which have a canonical set of instabilities that are manifest in practice.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
%\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
%\else
%  \DeclareGraphicsExtensions{.eps}
%\fi

\graphicspath{{figures/}{BrBuKaKu_SIAMReview/figures/}{BrBuKaKu_SIAMReview/}}
%strongly recommended
\numberwithin{theorem}{section}

% Declare title and authors, without \thanks
%\newcommand{\TheTitle}{Modern Koopman Operator Theory\\ for Data-Driven Dynamical Systems}
\newcommand{\TheTitle}{Modern Koopman Theory for Dynamical Systems}
\newcommand{\TheAuthors}{S. L. Brunton, M. Budi\v{s}i\'{c}, E. Kaiser, J. N. Kutz}

% Sets running headers as well as PDF title and authors
\headers{\TheTitle}{\TheAuthors}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{{\TheTitle}\thanks{Submitted to the editors Feb. 24, 2021.
\funding{
SLB acknowledges support from the Army Research Office (W911NF-17-1-0306 and W911NF-19-1-0045).
SLB and JNK acknowledge support from the Defense Advanced Research Projects Agency (DARPA contract HR011-16-C-0016) and the UW Engineering Data Science Institute, NSF HDR award \#1934292.
}}}

% Authors: full names plus addresses.
\author{
  \hspace{-.1in}Steven L. Brunton\thanks{Dept. of Mechanical Engineering, University of Washington, Seattle, WA (\email{sbrunton@uw.edu}).}
  \and
    Marko Budi\v{s}i\'{c}\thanks{Dept. of Mathematics, Clarkson University, Potsdam, NY (\email{mbudisic@clarkson.edu}).}
  \and
    Eurika Kaiser\thanks{Dept. of Mechanical Engineering, University of Washington, Seattle, WA  (\email{eurika@uw.edu}).}
  \and
  J. Nathan Kutz\thanks{Dept. of Applied Mathematics, University of Washington, Seattle, WA (\email{kutz.edu}).  \hspace{-.1in}}
}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}




%%% Local Variables:
%%% mode:latex
%%% TeX-master: "main"
%%% End:

